Non-idempotent intersection types and strong normalisation

We present a typing system with non-idempotent intersection types, typing a term syntax covering three different calculi: the pure {\lambda}-calculus, the calculus with explicit substitutions {\lambda}S, and the calculus with explicit substitutions, contractions and weakenings {\lambda}lxr. In each of the three calculi, a term is typable if and only if it is strongly normalising, as it is the case in (many) systems with idempotent intersections. Non-idempotency brings extra information into typing trees, such as simple bounds on the longest reduction sequence reducing a term to its normal form. Strong normalisation follows, without requiring reducibility techniques. Using this, we revisit models of the {\lambda}-calculus based on filters of intersection types, and extend them to {\lambda}S and {\lambda}lxr. Non-idempotency simplifies a methodology, based on such filter models, that produces modular proofs of strong normalisation for well-known typing systems (e.g. System F). We also present a filter model by means of orthogonality techniques, i.e. as an instance of an abstract notion of orthogonality model formalised in this paper and inspired by classical realisability. Compared to other instances based on terms (one of which rephrases a now standard proof of strong normalisation for the {\lambda}-calculus), the instance based on filters is shown to be better at proving strong normalisation results for {\lambda}S and {\lambda}lxr. Finally, the bounds on the longest reduction sequence, read off our typing trees, are refined into an exact measure, read off a specific typing tree (called principal); in each of the three calculi, a specific reduction sequence of such length is identified. In the case of the {\lambda}-calculus, this complexity result is, for longest reduction sequences, the counterpart of de Carvalho's result for linear head-reduction sequences.

==> CxLambdaS.tex <==
\subsection{$\LambdaS$}

In $\LambdaS$, we take advantage of the fact that $\Rew{W}$ can be postponed \wrt to $\Rew{B,S}$ steps.  This allows us to concentrate on $\Rew{B,S}$ and the normal forms for it.

\begin{lemma}[Refined Subject Reduction]
  If $\Deriliopt[n] \Gamma M A$ then:
  \begin{itemize}
  \item If $M \Rew{B} M'$, then there exist $\Gamma'$ and $m$ such that $\Gamma \approx \Gamma'$, $m<n$ and $\Deriliopt[m] {\Gamma'} {M'} A$
  \item If $M \Rew{S} M'$, then there exists $\Gamma'$ such that $\Gamma \approx \Gamma'$ and $\Deriliopt[n] {\Gamma'} {M'} A$
  \end{itemize}
  Moreover the degree of the typing tree does not change, and the principality property is preserved.
\end{lemma}
\begin{proof}
  We simply check that, in the proof of of Subject Reduction (Theorem~\ref{th:SubjectReduction-lS}), the optimality property, the degree and the principality property are preserved, as already mentioned in the proof of Subject Expansion (Theorem~\ref{th:SELambdaS}).
\end{proof}


\begin{toappendix}
  \appendixbeyond 0
  \begin{lemma}[Most inefficient reduction]
\label{lem:MostInefficientReduction}
    Assume $\Deriliopt[n] \Gamma M A$.
    If $M$ can be reduced by $\Rew{B}$ and not by $\Rew{S}$, then there exist $M'$ and $\Gamma'$ such that $\Gamma \approx \Gamma'$, $M \Rew{B} M'$ and $\Deriliopt[n - 1] {\Gamma'} {M'} A$.
  \end{lemma}
\end{toappendix}


\begin{toappendix}
  [\begin{proof} Again, we adapt the proof of Subject Reduction (Theorem~\ref{th:SubjectReduction-lS}). More precisely, see appendix \thisappendix.\end{proof}]
  \begin{proof}
    We follow the induction given in the proof of Subject Reduction (Theorem~\ref{th:SubjectReduction-lS}).
    In this induction, $n$ can be decreased by more than $1$ by a $\Rew{B}$ in two cases:
    \begin{itemize}
    \item In the case where the type is an intersection, then $n$ will be decreased by at least $2$.
    \item When we build a typing of $\Subst M x N$ from a typing of $(\l x . M) N$: if there were subsumption in the typing the $\l$-abstraction, then the proof calls Lemma~\ref{lem:basicprop}.4 which might decrease $n$ by more than $1$.
    \end{itemize}
    Those two cases are never encountered when optimality is assumed, as we prove the result by induction on $M$.
    Since $M$ cannot be reduced by $\Rew{S}$, it is of one of the following forms:
    \begin{itemize}
    \item $\l x . M_1$. It is clear that $M_1$ satisfies the necessary conditions to apply the induction hypothesis.
    \item $(\l x . M_1) N_1 \ldots N_p$ (with $p\geq 1$). We reduce to $\Subst{M_1} x{N_1}\ N_2\ldots N_p$.
      By the optimality property, $A$ is not an intersection, and none of the types of $((\l x . M_1) N_1\ldots N_i)_{1\leq i\leq p-1}$ are intersections either (since they are applied to an argument).
      Also by the optimality property, there is no subsumption in the typing of the $\l$-abstraction, and therefore the call to Lemma~\ref{lem:basicprop}.4 is replaced by a call to Lemma~\ref{lem:basicprop}.4 and therefore $n$ is decresed by exactly $1$.
    \item $\Subst {\Subst x {y_1} {N_1} ...} {y_p} {N_p} N_{p + 1} ... M_m$.
      Therefore there exists $i$ such that $N_i$ can be reduced by $\Rew{B}$. Moreover, optimality requires the type of $x$ to be of the form $A^+_1\arr \cdots\arr A^+_p\arr B-$, and therefore the sub-derivation typing $N_i$ is also optimal: we can apply the induction hypothesis on it.
    \end{itemize}
  \end{proof}
\end{toappendix}

\begin{lemma}[Resources of a normal term]\strut
  \label{lem:normalLambdaS}
  If $\Deriliopt[n] \Gamma M A$, and $M$ cannot be reduced by $\Rew{B, S}$, then
  $n$ is the number of applications in $M$.

	Moreover, if the typing tree is principal, then $n$ is the degree of the
typing tree.
\end{lemma}

\begin{proof}
  Straightforward.
\end{proof}

\begin{theorem}[Complexity result]
  If $\Deriliopt[n] \Gamma M A$, then $n = n_1 + n_2$ where
  \begin{itemize}
  \item $n_1$ is the maximum number of $\Rew{B}$ in a $B,S$-reduction sequence from $M$
  \item $n_2$ is the number of applications in the $B,S$ normal form of $M$.
  \end{itemize}
Moreover, if the typing tree is principal, then $n_2$ is the degree of the
typing tree.
\end{theorem}

\begin{proof}
  The previous lemmas give us a $B,S$-reduction sequence with $n - n_2$ $B$-steps, from $M$ to the normal form of $M$.  In this reduction sequence every reduction $B$ decreases the measure of the typing tree by exactly one.

  Assume we have a $B,S$-reduction sequence, from $M$ to the normal form of $M$ ($\LambdaS$ is confluent), with $m$ $B$-steps. By Subject Reduction (Theorem~\ref{th:SubjectReduction-lS}), the measure of the derivation typing the normal form of $M$ is smaller than $n-m$, but is also $n_2$.  Hence $m \leq n-n_2$.
  
  Assume we have a $B,S$-reduction sequence, from $M$ to any term $M_1$. It can be completed into a $B,S$-reduction sequence with more $B$-steps, from $M$ to the normal form of $M_1$.
\end{proof}



==> Dupl.tex <==
\subsection{Number of duplications}

\label{sec:other-inter}

By measuring the number of use of the Intersection rule in the typing tree
we get a bound on the number of duplications (the number of use of rules that
duplicate a term).

However, contrary to the other measures, we cannot have an equality result.

Here is a counter example :

\[(\l x . x x)(\l y . a y y)\]

If we reduce this term to its normal form we have two duplications.
However, if we type this term, we have at least 3 uses of the intersection
rule.

